Restoration of Fragmentary Babylonian Texts Using Recurrent Neural Networks

The main source of information regarding ancient Mesopotamian history and culture are clay cuneiform tablets. Despite being an invaluable resource, many tablets are fragmented leading to missing information. Currently these missing parts are manually completed by experts. In this work we investigate the possibility of assisting scholars and even automatically completing the breaks in ancient Akkadian texts from Achaemenid period Babylonia by modelling the language using recurrent neural networks.

==> sections/method.tex <==
  TOOO TODO TODO TOOO TODO TODO TOOO TODO TODO
TOOO TODO TODO TOOO TODO TODO TOOO TODO TODO
TOOO TODO TODO TOOO TODO TODO TOOO TODO TODO

